Noncompliance in randomized control trials without exclusion restrictions

This study proposes a method to identify treatment effects without exclusion restrictions in randomized experiments with noncompliance. Exploiting a baseline survey commonly available in randomized experiments, I decompose the intention-to-treat effects conditional on the endogenous treatment status. I then identify these parameters to understand the effects of the assignment and treatment. The key assumption is that a baseline variable maintains rank orders similar to the control outcome. I also reveal that the change-in-changes strategy may work without repeated outcomes. Finally, I propose a new estimator that flexibly incorporates covariates and demonstrate its properties using two experimental studies.

==> thesis_Application.tex <==
\section{Application}

%\paragraph{Question}
\subsection{Microcredit experiment in Morocco: background}

\cite{CreponDevotoDufloPariente2015} conducted a one-sided noncompliance experiment in the rural areas of Morocco, choosing target areas where the participant villagers had not experienced microcredit services before the experiment. This location choice was a novel feature of the study, and the authors estimated the relative effects of new access and no access, rather than the effect of expanding microcredit. Here, as introduced in Section 3, $T$ denotes the binary assignment (i.e., access to microcredit services) and D is the binary treatment of taking up microcredit. By construction, people in control villages, $T = 0$, automatically have $D = 0$. The administrative observation of the take-up decision validates the successful implementation of this procedure. Overall, the take-up rate is relatively low. As reported in column (1) of Table 2 in \cite{CreponDevotoDufloPariente2015}, only $16.8$\% of the treated units in the sample took a loan from the microcredit company. This number reduces to $14.3$\% with non-zero business outputs in the baseline survey.

For the present analysis, the most important feature is that \cite{CreponDevotoDufloPariente2015} conducted a detailed baseline survey before the experimental intervention. The dataset comprised the production output market values before and after the experiment. Although this baseline survey feature is common in field experiments, only a few studies allow the application of my strategy, as they do not report take-up behaviors in the baseline sample. Based on the aforementioned information, $Y_b$ denotes the baseline sales value output and $Y = T Y(1) + (1 - T)Y(0) = T(DY(1,1) + (1 - D)Y(1,0)) + (1 - T)Y(0)$ indicates the endline sales value output.

In the experiment, a local microfinance institution called Al Amana entered randomly selected villages. After Al Amana opened new branches at the beginning of the study, the authors conducted a baseline survey containing all the outcome measures of interest as the terminal outcome measures. Upon completing the baseline survey, a randomization process separated $162$ villages into $81$ pairs with similar observed characteristics; one of each pair was randomly assigned as the treatment village and the other as the control village. Al Amana agents visited the treatment villages and promoted participation in microcredit, while the control villages had no access. At the time of intervention, all the newly opened branches offered fully functional services. For the control group, we can confirm that this one-sided noncompliance feature, in the administrative report of the proportion of Al Amana clients, is zero. The main sample in \cite{CreponDevotoDufloPariente2015} is only a subsample (not the entire sample) of units that had a high borrowing probability. Although the study collected baseline survey observations for $4,465$ households, from $162$ villages, they also added the endline observations, totaling $4,934$ observations, as their analysis did not necessarily require a baseline survey structure. I use their extended sample in column (1) of Tables \ref{tbl:originalITT} and \ref{tbl:originalIV} to replicate their original estimates, but I limit the sample to the baseline survey units in the remainder of the study.

\begin{table}[tbh] 
 \caption{Intention-to-treat effects on business outcomes} 

 \label{tbl:originalITT}
 \centering
 \begin{tabular}{lcccc}
 \hline
 & (1) & (2) & (3) & (4)\\
Model & OLS & OLS & OLS & OLS\\ \cline{2-5}
Outcome & \multicolumn{2}{c}{level output} & \multicolumn{2}{c}{log output}\\ \hline
  Assignment ($T$) & $6,061^{***}$ & $5,889^*$ & $0.32^{***}$ & $0.37$\\
            & ($2,167$) & ($3,039$) & ($0.12$) & ($0.25$)\\
  \hline
  Self-employed in baseline &      & Y & Y & Y\\
  Strata dummies & Y & Y & Y & \\
  Obs       & $4,934$ & $2,453$ & $2,453$& $2,453$\\
  control mean & $30,450$ & $33,554$ & $8.71$& $8.71$\\
  %control median & 6,960 & 9,796 & 9.8829\\
  \hline
 \end{tabular}
 \vspace{0.3cm}
\begin{minipage}{325pt}
{\flushleft
 \fontsize{9pt}{9pt}\selectfont \smallskip NOTE: Standard
 errors reported in parenthesis are clustered in
 village levels. *, ** and *** indicate statistical significance of
 10\%, 5\%, 1\% sizes respectively. Units in levels are Moroccan Dirham,
 1MAD $\approx $ $0.11$ USD. Self-employed indicates that the estimates
 are for the subgroup of business owners at the baseline. %$\dagger$: inverse hyperbolic sine
 %transformation, $log(x + \sqrt{x^2 + 1})$, is applied instead of the
 %log to prevent ill-defined value for output value equals to zero.
 } %One observation with an extreme value of revenue in treatment
 %group is removed.}
\end{minipage}
\end{table}


Table \ref{tbl:originalITT} shows the ITT estimates using regression analysis to control for the covariates, including number of household members, number of adults, the household head's age, indicator variables for animal husbandry, other nonagricultural activities, outstanding loans over the past 12 months, household spouses as the survey respondents, and other household members acting as the survey respondents. These linear regression analyses are also conditioned for strata dummies (paired villages) except for column (4). 

As column (1) shows, there is a positive and significant effect of microcredit access on production output sales. As my method requires a continuous $Y_b$, I restrict the study sample to individuals who had positive sales values in the baseline survey. As emphasized earlier, $Y(0)$ and $Y(1)$ do not need to be continuous. Conditional on $Y_b > 0$, some observations with $Y = 0$ represent exit behaviors during the study period, and the mass at $Y = 0$ does not hamper the analysis.

This sample selection may change the interpretation of the effect but does not generate any bias. Columns (2) and (3) show the same estimates, except for self-employed individuals at the baseline. This procedure reduces the original sample size to approximately half. Column (2) shows the effect on the output level and column (3) shows the effect on the output log. As the output values contain zeroes, I apply the inverse hyperbolic sine transformation, $log(x + \sqrt{x^2+ 1})$, instead of the natural log. Therefore, the estimates interpret the approximated semi-elasticities for small effects. Overall, we need to convert the estimates using the hyperbolic sine formula to interpret the large coefficients, whereas the standard exponential approximation works well for this application to evaluate large means (for a detailed discussion, see \citealp{BellemareWichman2018}). Both effects are positive and precisely measured, and the remainder of the arguments are all based on the log output, as the revenue distribution is heavily right skewed with a few outliers. It appears that the issue of outliers in the output values does not matter extraordinarily. Appendix D.3 presents additional results using the output level with or without trimming the extreme output values, which are consistent with the log output findings in the main analysis.

%\begin{table}[tbh]
% \caption{Quantiles of the outcome measures}
% \centering
% \begin{tabular}{l|ccc}
%  \hline \hline
%   & output & output & log output\\
%   & whole & subsample & subsample\\
%  \hline
%  \hline
%  min & 0 & 0 & 0\\
%  \hline
%  25\% & 505 & 1,816 & 8.198 \\
%  median & 6,960 & 9,706 & 9.883 \\
%  75\% & 26,412 & 30,238 & 11.010 \\
%  max & 1,387,053 & 1,231,900 & 14.717\\
%  \hline \hline
% \end{tabular}
%\end{table}
%\footnote{As the support of the level
%seems to be unbounded, the estimator based on distribution regressions
%of the levels of the output does not seem to work very well. This
%unbounded nature of the outcome appears in the violation of the compact
%support assumption. Instead, all the results are shown in the log
%transformation of the outcome values.} 

\begin{comment}
 
\subsection{Original use of the baseline survey}

\cite{CreponDevotoDufloPariente2015} report the baseline survey for
a similar purpose to mine. The purpose is to assess the heterogeneity
in the ITT of the access to microcredit by subgroups with particular take-up decision.
In particular, our shared concern is the possibility of the direct
effect of microcredit access for those who do not take up credit.

As I quoted earlier in example \ref{ex.micro.quote}, there are many reasons why the access to microcredit might have a
direct effect even though people do not take up credit. For example,
the promotion of the credit company might encourage small business owners to
continue their business. Because of the new access, the owners expect to have additional
credit available in the future even though they are not borrowing right now. 
The nature of the village level assignment also generates equilibrium effects and peer effects. 
The expanded credit use in the treatment village would alter the
interest rates of informal lending and product prices within the village as equilibrium realizations. 
Furthermore, nonborrowing people might receive transfers from relatives
and friends who succeed in their business due to borrowing, while these
people might also need to cover the payment for the debt of failing relatives.


The idea of the original study is to estimate the propensity to borrow
from microcredit using covariates from a baseline survey. In other
words, the parameter
\[
 E[Y_1 - Y_0|P(D = 1|W = w) = p] = E[Y_1 - Y_0|W \in W_{p}]
\]
is identified, where $W_p \equiv \{w \in \mathcal{W}: P(D=1|W=w) = p\}$.
With this parameter, one might test the following hypotheses
\begin{align*}
 H_{0}^{High} &: E[Y_1 - Y_0|P(D = 1|W = w) \geq p_H ] = 0,\\
 H_{1}^{High} &: E[Y_1 - Y_0|P(D = 1|W = w) \geq p_H ] \neq 0,  
\end{align*}
and
\begin{align*}
 H_{0}^{Low} &: E[Y_1 - Y_0|P(D = 1|W = w) < p_L ] = 0,\\
 H_{1}^{Low} &: E[Y_1 - Y_0|P(D = 1|W = w) < p_L ] \neq 0.
\end{align*}
Table \ref{tbl:originalHetero} shows the results in the original article based on a regression analysis. 
The results suggest that the units with top 30\% of the propensity score have a more substantial and significant effect, while the units with bottom 30\% have a small and insignificant effect. 

\begin{table}[tbh] 
 \caption{Heterogeneity by high/low propensities} 

 \label{tbl:originalHetero}
 \centering
 \begin{tabular}{cccc}
 Outcome: & output &    output & log output \\
 \hline
  & (1) & (2) & (3)\\
  \hline
  High 30\% & 15773.7*** & 13647.2** & 0.4736**\\
   & (4153.6) & (6095.3) & (0.1985)\\
  \hline
  Low 30\% & 646.6 & 1818.3 & 0.2739\\
   & (2701.1) & (4088.1) & (0.1900)\\
  \hline
  Sample selection &  & &\\
  Self-employed&      & Yes & Yes \\
  \hline
  \hline
  control mean & 30,450 & 33,554 & 8.7079\\
  %control median & 6,960 & 9,796 & 9.8829\\
  Obs       & 4,934 & 2,453 & 2,453\\
  \hline \hline
 \end{tabular}
 \vspace{0.3cm}
\begin{minipage}{325pt}
{\fontsize{9pt}{9pt}\selectfont \smallskip Note: Standard
 errors reported in parenthesis are clustered in
 village levels. *, ** and *** indicate statistical significance of
 10\%, 5\%, 1\% sizes respecively. Self-employed indicates that the estimates
 are for the subgroup of business owners at the baseline.} %One observation with extreme value of revenue in treatment
 %group is removed.}
\end{minipage}
\end{table}

However, testing $H_0^{HIGH}$ or $H_{0}^{LOW}$ do not necessarily relate the primary
interest of whether the direct effect exists and invalidate the use of
IV estimator. First, the event of the low propensity score $\{P(D = 1|W
= w) < p_L\}$ might be different from the event of no take-up under treatment $\{D = 0, T = 1\}$.
The subgroup of nonborrowers $(D = 0, T = 1)$ might be sorted on
unobservables by $D$, but the propensity score based strategy allows
sorting only on observables $W$. Second, as we see in the discussion of the identification section,
a small violation to the exclusion restriction might result in a large
magnitude of the bias in the ATT when the take-up probability is
low. Therefore, a small violation to the null $H_0$, which is not
detectable, might generate a huge bias in the ATT.
\end{comment}

Table \ref{tbl:originalIV} shows the original and additional IV estimates that are valid only if the direct effect for the treated is zero. Under the conventional assumption, the estimated ATT may overestimate the effect for the treated, implying that policymakers may be overly encouraged to promote microcredit services. Thus, I compare my preferred estimate for the ITTTA with these two-stage least squares (2SLS) ATT/ITTTA estimates. The 2SLS estimates in columns (2) and (3) include paired village dummies, following \citeauthor{CreponDevotoDufloPariente2015}'s (\citeyear{CreponDevotoDufloPariente2015}) original specification. For my later estimates, I do not include these paired village dummies to prevent the incidental parameters problem for nonlinear estimators. Nevertheless, the 2SLS estimate with dummies in column (4) has a similar magnitude to the estimate without dummies in column (3), indicating that strata dummies improve their precision.
\begin{table}[tbh] 
 \caption{ATT under assumption of no direct effect} 

 \label{tbl:originalIV}
 \centering
 \begin{tabular}{lcccc}
\hline
 & (1) & (2) & (3) & (4)\\
Model & 2SLS & 2SLS & 2SLS & 2SLS \\ \cline{2-5}
Outcome & \multicolumn{2}{c}{level output} & \multicolumn{2}{c}{log output}\\ \hline
  Treatment ($D$) & $36,253^{***}$ & $42,026^*$ & $2.29^{***}$ & $2.57$\\
            & ($12,494$) & ($21,525$) & ($0.85$) & ($1.71$)\\
  \hline
  Self-employed in baseline &      & Y & Y & Y\\
  Strata dummies & Y & Y & Y & \\
  Obs       & $4,934$ & $2,453$ & $2,453$  & $2,453$\\
  control mean & $30,450$ & $33,554$ & $8.71$ & $8.71$\\
  %control median & 6,960 & 9,796 & 9.8829\\
  \hline
 \end{tabular}
 \vspace{0.3cm}
\begin{minipage}{325pt}
{\flushleft
 \fontsize{9pt}{9pt}\selectfont \smallskip NOTE: Standard
 errors reported in parenthesis are clustered in
 village levels. *, ** and *** indicate statistical significance of
 10\%, 5\%, 1\% sizes respecively. Self-employed indicates that the estimates
 are for the subgroup of business owners at the baseline. 2SLS stands for the two-stage least squares method.
 } %One observation with extreme value of revenue in treatment
 %group is removed.}
\end{minipage}
\end{table}

\subsection{ITTTA and ITTNA estimations}

With the baseline outcome $Y_b$ as the proxy for the control outcome $Y(0)$,
I can directly identify the counterfactual distribution of $Y(0)$ conditional on the endogenous subgroup $\{T = 1, D = d\}$ for each $d \in \{0,1\}$ (see Section 3 for details of this procedure). 

Outcomes $Y_b$ and $Y(0)$ are the production output sales values stemming from small business activities. Based on the random assignment of credit access $T$ and the fact that microcredit was not available during the baseline period or for control villages, these two outcomes, $Y_b$ and $Y(0)$, should be similar, except for the random shocks occurring over the study's two-year period. Appendix C.4 offers detailed arguments to justify the rank similarity based on the so-called \textit{slippages} argument (\citealt{HeckmanSmithClements97}). In this study, although the rank similarity assumption does not have any testable restrictions per se, I conducted a diagnostic test supporting the rank similarity assumption in this application (see Appendix D.4 for results and other details).

%Suppose that the slippages $\tilde{U}_{b,w}$ and $\tilde{U}_{0,w}$, in the rank
%orders from the potential productivity ranking $U$
%do not depend on their counterfactual credit take-up decision $D$
%conditional on $U$. Then the rank similarity assumption might be justified. 

Table \ref{tbl:mainResults} shows the estimates of the subgroup effects
unconditional on $W$ achieved by integrating $W$ out.
Column (1) represents the ITTNA, the direct effect for the nontreated $D = 0$ with assignment $T = 1$. Column (2) addresses the ITTTA, as the combined effect of taking up treatment $D = 1$, with takers gaining access to assignment $T = 1$. In column (3), I offer a back-of-the-envelope calculation of the treatment's net effect, or the ATT, as discussed in Section 3.3.
\begin{table}[tbh]
 \centering
  \caption{Estimates with the baseline proxy $Y_b$} 

 \label{tbl:mainResults}
 \begin{tabular}{lccc}%c}
 % Method: & \multicolumn{2}{c}{Rank Similar} & 2SLS \\%& Unconditional \\
 %\hline
 \hline
 & (1) & (2) & (3)\\
Model & RS & RS & RS \\ 
Parameter & ITTNA & ITTTA & ITTTA - ITTNA \\ \cline{2-4}%& ATT \\%& ITT\\
Outcome & \multicolumn{3}{c}{log output}\\
  \hline
  Assignment ($T$) & $0.28$ & $1.03^{**}$ & $0.74^*$ \\%& 0.4569 \\
  by subgroups of ($D$)    & ($0.28$) & ($0.45$) & ($0.44$) \\%& \\
  \hline
  %exp(TE) - 1 & $0.33$ & $1.79$ \\ %& $8.92$ \\ %& 0.5792 \\
  %control mean & 8.7079 & 8.7079 & 8.7079\\
  %control median & 6,960 & 9,796 & 9.8829\\
  Self-employed in basline & Y & Y & Y\\
  Obs       & $2,453$ & $2,453$ & $2,453$ \\ %& $2453$  \\%& 2453 \\
  %\hline
  %Selection bias: & 0.034 & 0.110 &  0.133 \\
  %Selection bias: & -0.058 & -0.056 &  0.031 \\
  %predicted & & & \\
  \hline
 \end{tabular}
 \vspace{0.3cm}
\begin{minipage}{325pt}
{\flushleft
 \fontsize{9pt}{9pt}\selectfont \smallskip NOTE: Standard
 errors reported in parenthesis are generated from 300 bootstrap draws clustered in
 village levels for (1)-(3). *,**,*** indicates statistical significance of
 10\%,5\% and 1\% sizes respectively. Logit link is used for (1) and
 (2). RS stands for the rank similarity estimator proposed in this paper.
 } %2SLS in (3) uses the same set of covariates as in (1) and (2).}
\end{minipage}
\end{table} 

As shown in column (2), the ITTTA is strongly positive and significant, but its magnitude is less than $45$\% of the 2SLS estimate, which should have been similar to the ITTTA if the direct effect for the treated was zero. A cautionary note when interpreting the difference between the two point estimates for the treated is that it is not statistically significant. As the p-value of the test for this difference is $0.182$, it is not possible to conclude that the proposed estimate implies that the 2SLS estimator is biased. Indeed, this insignificance appears in column (1), as the ITTNA, representing the estimated direct effect for the nontreated, is insignificant. 
If the direct effects are homogeneous, then the magnitude and insignificance of the ITTNA may correspond to the magnitude and insignificance of the difference between the ITTTA and IV. By combining the ITTTA and ITTNA signs and magnitudes, $T$ may still have a positive direct but imprecisely estimated effect. Nevertheless, we cannot distinguish imprecisely estimated small effect against no effect.
 %\footnote{They are not precisely comparable to the estimate in (2) is the unconditional subgroup effect, while the estimate in (3) is the conditional subgroup effect from the regression analysis. Nevertheless, the unconditional ATT by integrating out the covariates produces higher magnitudes which instead reinforces the issue I raise here.}
%This direct effect estimate itself is
%similar to the magnitude of the low propensity group estimate in Table
%\ref{tbl:originalHetero} of column (3).

Column (3)'s ATT back-of-the-envelope calculation suggests a sufficiently large effect from the treatment itself. Although the validity of this estimate depends on the homogeneity of the direct effect, the direct effect may be smaller for the treated than the nontreated, as discussed in Section 3.3. Therefore, it is assuring to see the positive and marginally significant effect confirming the ATT's positivity. In Appendix D.1, I display the quantile differences of the direct effects for the nontreated, $D = 0$, (Figure 1) and the quantile difference of the combined effects for the treated, $D = 1$, (Figure 2), along with uniform $95$\% confidence intervals. The results indicate the relatively monotonous effects over the range of quantile values for the combined effect of the treated. Specifically, the quantile differences are conditional on those who had businesses at the baseline. Therefore, this result does not contradict previous findings that business revenue effects appear in the upper tail of the distributions (\citealp{AngelucciKarlanZinman15}).

Although Table \ref{tbl:mainResults} findings may alter policymakers' decisions, I must clarify two limitations of this analysis. First, the focus of this study was limited to the subsample of business owners before the experiment. Second, the conventional IV estimate and my preferred estimate differ, but not statistically. Therefore, my empirical results should be considered as additional evidence for policymakers. I encourage future researchers to collect a detailed baseline survey to evaluate the intervention of interest and further understand the nature of the treatment effect through the ITTTA and ITTNA.

%\paragraph{Data}

%\paragraph{Results}

==> thesis_Estimation.tex <==
\section{Estimation}

As demonstrated in Section 3 and Appendix C.4, it is desirable to condition the distributions on pretreatment covariates $W$ to justify the conditional rank similarity. Dimensionality becomes a serious issue when we nonparametrically estimate conditional distribution functions for each subsample $\{T=1,D=d,W=w\}$, with W containing continuous variables. 
\cite{MellySantanglo15} extended \citeauthor{AtheyImbens06}' (\citeyear{AtheyImbens06}) estimator to incorporate covariates into a semiparametric quantile regression model. However, semiparametric quantile regressions remain flexible only when they involve a smooth conditional density (see \citealt{ChernozhukovFernandezValMelly13}).
As my identification analysis now accepts $Y(0)$ as a binary or discrete random variable, the quantile regression approach may be undesirable. Therefore, I consider a distribution regression-based approach and incorporate \citeauthor{DaveziesDHaultfoeuilleGuyonvarch18}'s (\citeyear{DaveziesDHaultfoeuilleGuyonvarch18}) recent development of cluster-robust inferences for the empirical process. Finally, cluster dependency is inevitable in my leading examples and my inference strategy closely follows that of \cite{ChernozhukovFernandezValMelly13}.

%Secondly, unlike
%\cite{MellySantanglo15} who employs quantile regressions all the way,
%distribution regressions attain the unconditional counterfactual mean
%$E[Y_0|T=1,D = d]$ by less number of inversions.\footnote{The case without covariates is
%estimated in a simpler form as analogy to \cite{AtheyImbens06}. The
%similar but different asymptotic distribution is shown in the appendix.}
%Nevertheless, the unconditional quantiles $Q_{Y_0|T=1,D =
%d}(\tau)$ are also attained by inverting the unconditional distribution
%functins $F_{Y_0|T=1,D = d}(y)$.

I begin with a random sample of observations. Consider an estimation of the semiparametric conditional distribution functions. To estimate the parameter of interest, I first estimate the following distribution functions:
\[
 F_{Y_b|T,W}(\cdot|1,w),F_{Y_b|T,W}(\cdot|0,w),\{F_{Y_b|T,D,W}(\cdot|1,d,w)\}_{d \in
\{0,1\}}.
\]
Hereafter, $W$ is a transformed vector of the original pretreatment covariates, such as polynomials or
B-splines, and $K$ is the set of indexes for the subgroups, such as $\{T = 1,
D = d\}$ or $\{T = 1\}$. Following \cite{ForesiPeracchi1995} and \cite{ChernozhukovFernandezValMelly13},
I estimate the conditional distribution functions for $Y$ conditional on a
subgroup $k$ out of $K \equiv \{\{T = 1\},\{T = 0\},\{T = 1,D = 1\}, \{T = 1, D = 0\}\}$ and $W$ as
\[
 \hat{F}_{Y|W,K}(y|w,k) = \Lambda (w'\hat{\beta}^{k}(y))
\]
for some known link function $\Lambda(\cdot)$. I estimate $\hat{\beta}(y)$ as
\begin{align*}
 \hat{\beta}^{k}(y) = \arg \max_{b \in \mathbb{R}^{dW}} \sum_{i = 1}^{n}&\left\{
 \left[I\{Y_i \leq y\}\log[\Lambda(W_i'b)] \right]\right.\\
 &+ \left.\left[I\{Y_i > y\}\log[1 - \Lambda(W_i'b)] \right]\right\}I\{K_i
 = k\}
\end{align*}
for each $y \in \mathcal{Y}^k$ where $\mathcal{Y}^k$ is the support of $Y$
conditional on the subgroup $k$ and $dW$ is a dimension of $W$. 
For the main application in Section 5, I use the logit link function. Appendix D.2 shows the robustness to other link function choices such as probit link and complementary log-log link. 

\begin{comment}
As an alternative, quantile function of $Y$ for $T = 1$ may be estimated
directly. Following the quantile regression estimator of \cite{KoenkerBassett78},
\[
 \hat{Q}_{Y|W,T}^1(\tau|w,1) = w'\hat{\beta}_{1}^Q(\tau)
\]
where
\[
 \hat{\beta}^{Q}_{1}(\tau) = \arg \min_{b \in \mathbb{R}^{dW}}
 \sum_{i=1}^n (\tau - I\{Y_i \leq W_i'b\})(Y_i - W'_i b).
\]
\end{comment}

Once these estimators are obtained, the conditional counterfactual
distribution is
\[
 \hat{F}_{Y(0)|W,T,D}(y|w,1,d) =
 \hat{F}_{Y_b|W,T,D}(\hat{Q}_{Y_b|W,T}(\hat{F}_{Y(0)|W,T}(y|w,0)|w,1)|w,1,d)
\]
where
\[
 \hat{Q}_{Y_b|W,T}(\tau|w,1) = \inf\left\{y \in \mathcal{Y}^{1,w}_b : \hat{F}_{Y_b|W,T}(y|w,1)
 \geq \tau \right\},
\]
in which $\mathcal{Y}_b^{1,w}$ is the support of $Y_b$ conditional on
$\{T = 1, W = w\}$ and $\tau \in [0,1]$ is a corresponding percentile. Therefore, the unconditional distribution can be obtained by
\[
 \hat{F}_{Y(0)|T,D}(y|1,d) = n_{1,d}^{-1}\sum_{i=1}^{n} \hat{F}_{Y(0)|W,T,D}(y|W_i,1,d)I\{T_i=1,D_i=d\}
\]
where $n_{1,d} \equiv \sum_{i} I\{T_i = 1,D_i=d\}$. The mean effect of
interest is obtained as follows
\[
 \hat{\mu}_d = \frac{1}{n_{1,d}} \sum_{i:T_i=1,D_i=d} Y_i  -
 \int_{\mathcal{Y}^0} y d\hat{F}_{Y(0)|T,D}(y|1,d)
\]
and the quantile difference is obtained by inverting the distribution functions
\[
 \hat{Q}_{Y(1)|T,D}(\tau|1,d) - \hat{Q}_{Y(0)|T,D}(\tau|1,d), \forall \tau \in (0,1).
\]

For the random sample of clusters, rather than individual
observations, I estimate
\[
 \hat{F}^C_{Y|W,K}(y|w,k) = \Lambda (w'\hat{\beta}^{C,k}(y))
\]
with
\begin{align*}
 \hat{\beta}^{C,k}(y) = \arg \max_{b \in \mathbb{R}^{dW}} &\sum_{c =
 1}^{\bar{C}}\sum_{i = 1}^{N_c}\left\{ \right.
 \left[I\{Y_{i;c} \leq y\}\log[\Lambda(W_{i;c}'b)] \right]\\
 &+ \left. \left[I\{Y_{i;c} > y\}\log[1 - \Lambda(W_{i;c}'b)] \right]\right\}I\{K_{i;c}
 = k\}
\end{align*}
for each $y \in \mathcal{Y}^k$, where $\bar{C}$ is the number of 
clusters and $N_c$ represents the size of each cluster $c$.
The difference appears in the bootstrap procedure and a few modifications under the assumptions of the data-generating process. In Appendices A.1 and A.2, I show that the proposed estimators are uniformly asymptotically normal. As a result, (clustered) exchangeable bootstrap inferences are shown to be valid for generating uniform confidence intervals (see also Appendices E.1 and E.2 for this estimator's finite sample properties).

==> thesis_Extension.tex <==
\section{Two-sided noncompliance}

Thus far, I have focused on one-sided noncompliance cases because two-sided noncompliance designs are complicated by the dynamic nature of taking up the treatment. This complication further distinguishes my analysis from the previous literature, including \cite{HuberSchelkerStrittmatter2019}, by selecting plausible kinds of latent rank restrictions separately for each design. In two-sided noncompliance cases, the practical complication involves justifications for the rank similarity assumption for which the rationale is that the underlying latent rank of the control outcome $Y(0)$ and proxy variable $Y_b$ would be similar conditional on the endogenous subgroups of $D$ and $T$. In one-sided noncompliance cases, the similarity of $Y(0)$ and $Y_b$ is a natural concept because both variables are determined when neither $T$ nor $D$ is available. For two-sided noncompliance designs, $Y(0)$ is no longer a purely comparable outcome with $Y_b$. As the control units may have taken up treatment $D$ without assignment $T$, $Y(0)$ represents the outcomes nontreated $D = 0$ and treated $D = 1$ under $T = 0$. Below, I articulate my argument for two-sided noncompliance designs in two cases.

If $D(1)$ and $D(0)$ denote the potential choice under assignment $T$, then $D = TD(1)+(1-T)D(0)$. A two-sided noncompliance experiment is a design $(Y,D,T)$ generated from $D(t) \in \{0,1\}$ for both $t \in \{0,1\}$. The observed outcome takes the following form: 
\begin{equation}
 Y = T (D(1) Y(1,1) + (1 - D(1))Y(1,0)) + (1 - T)(D(0) Y(0,1) + (1 -
  D(0))Y(0,0)) \label{eq:twoSided}
\end{equation}
where $Y(t,d)$ represents the outcome with assignment $T = t$ and treatment $D = d$.

The main parameters stay the same as the ITTTA and ITTNA. Under the monotonicity of $D(1) \geq D(0)$ almost surely, they have similar interpretations. The ITTTA is a principal stratification effect of $E[Y(1,1) - Y(0,D(0))|T = 1, D(1) = 1]$ for the union of basic principal stratum $\{D(1)=1,D(0)=0\} \cup \{D(1)=1,D(0)=1\}$. The ITTTA is also the sum of the effect from the intended channel for the complier, $E[(1 - D(0))(Y(1,1) - Y(1,0))|T = 1, D(1) = 1]$, and the assignment's direct effect for the treated holding the same treatment status in the control, $E[Y(1,D(0)) - Y(0,D(0))|T = 1, D(1) = 1]$. Therefore, verifying the ITTTA can still determine whether $T$ has an impact, at least for those who comply with intention $T$. The ITTNA is the same direct effect $E[Y(1,0)-Y(0,0)|T=1,D(1)=0] = E[Y(1,0) - Y(0,0)|D(1) = D(0) = 0]$ by monotonicity. Nevertheless, the identification rationale may differ.

%These differenes in the strength of the imposed models appear as a variety of parameters identified in \cite{HuberSchelkerStrittmatter2019} and a relatively few parameters identified in my paper. 

\subsection{Treatment available before the randomized assignment}

%For this case, I apply the same strategy as the onesided noncompliance, assuming that the treatment takeup $D$ is \textit{stable} over time as considered in \citet[Assumption 2]{deChaisemartinDHaultfoeuille2017} .

%For the case of $D_1 \geq D_0$ almost surely, consider $d = 0$. The
%modified assumption states that the latent rankings defined for the
%subgroup of $\{T = 0, D = 0\} = \{D_0 = 0\}$ under randomization
%assumption \ref{ass:CIZ} have the same distributions conditional on
%its further subgroup of $\{D_0 = 0, D_1 = 0\}$.

Consider a two-sided noncompliance experiment where treatment $D$ may be available before the assignment of $T$. If the same treatment $D$ had been available in a previous period, but assignment $T$ encouraged taking up $D$, then the rank similarity strategy for one-sided noncompliance cases may still work out. Nevertheless, the justification for Assumption \ref{ass:RS} should be based on $Y(0,1)$ and $Y(0,0)$, instead of $Y(0)$. The key notion is the stability of taking up treatment $D$ within the units without the assignment. While $D$ was available in the baseline, no factors should affect take-up behavior $D$ in the control group $T = 0$. Therefore, the $D$ distribution should not change in the control group over time. If $D_b$ is the treatment in the baseline and $Y_{b}(0)$ and $Y_{b}(1)$ are the baseline proxies with and without $D_b$, then $Y_b \equiv Y_{b}(1)D_b + Y_{b}(0)(1 - D_b)$. With these notations, I propose the following modified rank similarity assumption.
\begin{assumption} \label{ass:RSTS}
 Suppose that Assumption \ref{ass:overlapSpp} holds for the simplicity.
 Then, $U_{b,d,w}$ is the latent ranking of $Y_{b}(d)$ for $d \in \{0,1\}$, and $U_{0,d,w}$ is the
 latent ranking of $Y(0,d)$ for $d \in \{0,1\}$, as defined in Definition \ref{def:latentRank}. This allows us to assume that
 \[
  P(U_{b,d,w} \leq u|W=w, D(1)= d', D_b = d) = P(U_{0,d,w} \leq u|W=w, D(1)= d', D(0) = d)
  %U_{b,d,w} \sim U_{0,d,w} | W=w, D(1)= d', D(0) = d)
 \] 
 for each $(d,d') \in \{0,1\}^2, w \in \mathcal{W}$.
\end{assumption}
%Note that one can construct $U_{0,d,w}$ from the distribution functions of $Y(0,d)$ as in Section 3, and the contruction yields the latent rank of $U_{0,w}$ for $Y(0)$ because the construction is linear in distribution functions 
This modified rank similarity imposes that the latent rankings do not change in $Y(0,d)$ and $Y_{b}(d)$ for those who maintained the same treatment status $D(0) = D_b = d$ without assignment $T = 0$, and who would behave similarly in $D(1)$. With this modified rank similarity, the ITTTA and ITTNA are identified when the compliance rates are \textit{stable} over time without the assignment (see \citealt{deChaisemartinDHaultfoeuille2017}, Assumption 2).
\begin{corollary} \label{cor:RSTS}
  Suppose that Assumptions \ref{ass:WDP}, \ref{ass:CIZ}, \ref{ass:UQ},
 \ref{ass:overlapSpp} and \ref{ass:RSTS} hold. Furthermore, assume that
 \[
  P(D(0) = 1|D(1) = d, W = w) = P(D_b = 1|D(1) = d, W=w)
 \]
 for each $d \in \{0,1\}$ and $w \in \mathcal{W}$, and $D(1) \geq D(0)$ almost surely. Then, we have
 \[
  F_{Y(0)|W,T,D}(y|w,1,d) = F_{Y_b|W,T,D}(Q_{Y_b|W,T}(\tau_{y,w}|w,1)|w,1,d), \tau_{y,w} \equiv F_{Y(0)|W,T}(y|w,0)
 \]
 for every $d \in \{0,1\}, w \in \mathcal{W}$ and $y$ in the support of $Y(0)|W=w,D=d$.
\end{corollary}
\begin{proof}
 From Lemma C.1 in Appendix C.1, Assumption \ref{ass:RS} holds for $Y(0) = Y(0,1)D(0)  + Y(0,0)(1 - D(0))$. The proof concludes by satisfying all the conditions for Theorem \ref{thm:IdRS}.
\end{proof}

\subsection{Two-sided noncompliance, but not before the experiment}

%For example, the models in \cite{DeuchertHuberSchelker2018} and \cite{HuberSchelkerStrittmatter2019} can be seen as $T$ and $D$ are not available in the baseline. 
Next, I consider treatment $D$ introduced after assignment $T$. In this case, it is difficult to justify the rank similarity in an analogous manner. While $Y(0)$ now contains the outcome of taking up treatment $D$, $Y_b$ cannot have this component in the baseline. Thus, I consider a modification to the rank similarity to deal with this difficulty. The weakened rank similarity assumption imposes a restriction only for the nontreated, solely restricting on the latent ranks of $Y(0,0)$ and $Y_b$ given $D = 0$ and $T = 0$.
%Formally speaking, I modify the rank similarity assumption to the following:
\begin{assumption} \label{ass:RSTS2}
  Suppose that Assumptions \ref{ass:WDP}, \ref{ass:CIZ} and \ref{ass:overlapSpp}, $D(1) \geq D(0)$ almost surely, and for every $w \in
 \mathcal{W}$, $(U_{b,0,w},U_{0,0,w})$ represents the latent rankings of $Y_b$ and $Y(0,0)$ conditional on $T = 0, D
 = 0, W = w$, then we can assume that
 \[
  %\tilde{U}_{b,0,w}|D(1) = 0, D(0) = 0, W = w \sim \tilde{U}_{0,0,w}|D(1) = 0, D(0) = 0, W = w.
  U_{b,0,w} \sim U_{0,0,w}|D(1) = 0, D(0) = 0, W = w.
 \]
\end{assumption} 
Given this weaker restriction, I show the ITTNA identification process, but not for the ITTTA.
\begin{theorem} \label{thm:twosidedID} 
 Suppose that Assumptions \ref{ass:RSTS2} and \ref{ass:UQ} hold, with the distribution of $Y_b$ being conditional on $\{T = 0, D = 0, W = w\}$ for every $w \in \mathcal{W}$. Then,
 \begin{align*}
  %&F_{Y(0)|D(1)}(y|0)\\
 &F_{Y(0)|D,T}(y|0,1)\\ 
 &= \int
 F_{Y_b|D,T,W}(Q_{Y_b|D,T,W}(F_{Y(0,0)|D ,T,W}(y|0,0,w)|0,0,w)|0,1,w)dF_{W|D,T}(w|0,1)  
 \end{align*}
and therefore, we identify $E[Y(1) - Y(0)|D = 0, T = 1] = E[Y(1,0) - Y(0,0)|D(1)=0].$
\end{theorem}
\begin{proof} 
 See Appendix B.
\end{proof}
%\begin{remark}
% Note that the monotonicity is sufficient but not necessary for the
% identification of the subgroup effects. I can weaken the monotonicity assumption
% into the following assumptions
% \[
%  P(Y_b \leq y|D_1 = 0) = P(Y_b \leq y|D_1 = 0,D_0 = 0)
% \]
% and
% \[
%  P(Y_{0} \leq y|D_1 = 0) = P(Y_{00} \leq y|D_1 = 0,D_0 = 0).
% \]
% See these statements are in fact necessary conditions for the
% monotonicity in the appendix lemma \ref{lmm:MonoFact}.
%
% These statements may be useful for treatments which has not been
% available in the baseline. Monotonicity requires that there is no defier. On the other hand, the
% above assumptions allow defiers but requires the defier and the
% never-taker have the same marginal distribution of $Y_b$ and
% $Y_{0}$. One possibility is the differences in defier and never-taker
% appear just because of random shocks which are independent of
% outcomes. Still the statement for $Y_0$ may be hard to justify in a
% general context. In the later section of differential attrition
 %example, I demonstrate that these alternatiev representation may be
 %useful alternative to the monotonicity.
%\end{remark}

The ITTTA may still be identified from the total law of expectation using the ITT estimate. In other words, $ITTTA = ITT - ITTNA \times \frac{P(D=0|T = 1)}{P(D=1|T = 1)}$. Nevertheless, it is limited in its precision when it must be divided by the small probability of $P(D = 1|T = 1)$ if the take-up rate is low. In addition, the ITTNA can be the only parameter of interest in some two-sided noncompliance designs. In Appendix C.4, I provide an example of the selective attrition problem, which is illustrated with \cite{vandenBergVikstrom2014}, to show the usefulness of Theorem \ref{thm:twosidedID} on its own.

%The above theorem identifies the control outcome distribution for
%the never-takers allowing us to identify the ITTNA, $E[Y(1) - Y(0)|T = 1, D(1)=0]$. However, we do not have the same formula for the ITTTA, unlike the previous two-sided noncompliance Corollary \ref{cor:RSTS}. 

% The stated formula in this case is numerically
%equivalent to the one stated in \cite*{HuberSchelkerStrittmatter2019}
%when outcomes in two periods are both continuously distributed. On the
%one hand, \cite*{HuberSchelkerStrittmatter2019} assume continuous outcomes in two
%periods and exploit the inverse of the distribution function of the post-intervention
%outcomes to produce the counterfactual quantile directly. On the other hand, I do not assume the continuity of the
%outcome by not inverting the distribution function of the
%post-intervention outcome to produce the counterfactual distribution.

%While the rank similarity may be rationalized in both cases of (i)
%introducing treatment which has not been available and (ii) stable
%control group, the former case might be difficulty to rationalize when
%there is some changes other than the intervention occurs in the control
%group. One exceptional case is the attrition problem.

%from the monotonicity, and there is no role of the homogeneous direct
%effect. Finally, assume we have baseline observation $Y_b$ for the proxy
%of $Y_0$. Let $F_{Y|W}^{0*}(\cdot|w)$ denote the conditional
%distribution function of $Y_0^*$.
\begin{comment}
\begin{corollary} 
 Consider the differential attrition model
 $(Y_{1}^*,Y_{0}^*,D_1,D_0,W,Y_b)$ as specified above. Suppose
 assumptions \ref{ass:WDP}, \ref{ass:CIZ}, and \ref{ass:overlapSpp} hold
 and, assumption \ref{ass:UQ} holds for a baseline variable $Y_b$
 conditional on $W,T = 0, D = 1$. Let $U_{b1}$ be the latent ranking of $Y_b$ conditional on $T = 0, D = 1, W = w$.

 Suppose further that assumption \ref{ass:RSTS2} with $d = 1$, and the
 monotonicity in the form of $D_0 \geq D_1$ almost surely holds. Then
 \[
  F_{Y|D = 1,T = 1}^{0*}(y) = \int
 F_{Y|D=1,T = 1,W}^b(Q_{Y|D=1,T = 0,W}^b(F_{Y|D = 1,T =
 0,W}^{0*}(y|w)|w)|w)dF_{W|D = 1, T = 1}(w)
 \]
 so that we have identification of
 \[
  E[Y_1^* - Y_0^*|D_1 = 1].
 \]
\end{corollary}
\begin{proof}
 The proof immediately follows as a special case of theorem \ref{thm:twosidedID} by flipping the order of the monotonicity from $D_1 \geq D_0$ to $D_0 \geq D_1$, and focused on the case of $D_1 = 1$ which implies $D_0 = 1$ almost surely.
\end{proof}
\begin{remark}
% As in the case of two-sided noncompliance, the conditional independence statements
% \[
%  P(Y_b \leq y|D_1 = 1) = P(Y_b \leq y|D_1 = 1,D_0 = 1)
% \]
% and
% \[
%  P(Y_0 \leq y|D_1 = 1) = P(Y_0^* \leq y|D_1 = 1,D_0 = 1)
% \]
% are sufficient for the identification. In fact, for the differential
% attrition, these restrictions may be substantially weaker than the
% monotonicity. 

%Because the former may allow shocks to $D_0$ conditional
% on $D_1 = 1$ which are independent from $Y_b$ and $Y_0^*$, the monotonicity
% may be violated. On the other hand, the violation to the monotonicity
% would not create the complication because the (inputation) value of the
% attrition is known to be the lowerest ranking.

The same approach may not work if the differential attrition works in the other way, namely $D_1 \geq D_0$. Nevertheless, if we may assume the rank similarity in $U_b$ and $U_{1}^*$ conditional on $T = 1, D = 1, W = w$, then the same argument works to identify
\[
 E[Y_1^* - Y_0^*|D_0 = 1].
\] 
\end{remark}
\end{comment}

\subsection{Identifying other parameters}
The limited identifiability in Theorem \ref{thm:twosidedID} derives from the restriction's weakness, which is typical of a two-sided noncompliance design. Further, the proposed rank similarity approach itself cannot identify the other parameters studied in \cite{HuberSchelkerStrittmatter2019}, such as the net (indirect) effects of $D$ for the compliers or other principal strata. The critical difference lies in their restrictions on the model. As with other CiC models, \cite{HuberSchelkerStrittmatter2019} assumed that the potential outcomes $Y(t,d)$ share a common latent rank variable across $(t,d) \in \{0,1\}^2$. Given that the same single unobserved scalar governs all the outcomes with and without assignment $T$ within a strong model, the restrictions on the common latent variable allow them to identify all the mediation parameters. \cite{HuberSchelkerStrittmatter2019} successfully found the mechanical latent rank conditions needed for each mediating effect, but the rationales for each latent rank restriction is not provided. Specifically, for operations involving the treated outcomes $Y(1)$, it is challenging to justify the associated latent rank restrictions. Further, it is difficult to weaken \cite{HuberSchelkerStrittmatter2019} restrictions because the latent rank restrictions are not separated from the model.

In this study, I do not impose such a model, but the potential outcome structure. With only the potential outcome structures, I explicitly declare which latent rank restrictions could be plausible under what kinds of designs, thereby offering a conservative approach to identifying the key principal stratification parameters. Nevertheless, I consider the net effects of treatment $D$, which is the ATT, with a homogeneity assumption rather than the latent rank restrictions for $Y(1,0)$ or $Y(1,1)$, as shown in Section 3.3. A similar procedure is possible in two-sided noncompliance designs. In Appendix C.2, I describe the identification process of the following \textit{net} effect of $D$ for the complier, similar to the local average treatment effect (LATE):
\begin{align}
 E[Y(0,1) - Y(0,0)|D(1) > D(0)] = (ITTTA - ITTNA)\frac{E[D(1)]}{E[D(1)] - E[D(0)]}\label{eq:LATE}
 %E&[Y(1,1) - Y(1,0)|T = 1, D(1) > D(0)] = (ITTTA - ITTNA)\frac{E[D(1)]}{E[D(1)] - E[D(0)]} \label{eq:LATE}\\
 %E&[Y(0,1) - Y(0,0)|T = 1, D(1) = 1] = ITTTA - \left(\frac{E[D(0)]^2}{E[D(1)]}\right)ITTNA \label{eq:LATE}
\end{align}
under a homogeneity assumption, $E[Y(1,1)-Y(0,1)|D(1) = 1] = E[Y(1,0) - Y(0,0)|D(1) = 0]$, that is stronger than that discussed in Section 3.3. The formula follows because $ITTNA = E[Y(1,0) - Y(0,D(0))|D(1) = 0] = E[Y(1,0) - Y(0,0)|D(1) = 0]$ when $D(1) \geq D(0)$ almost surely. As in Section 3.3, the above net effect may still work as a back-of-the-envelope calculation when the homogeneity assumption is violated. (see Appendix F for the empirical application of two-sided noncompliance and homogeneity assumption justifications).

%which shares a similarity to the local average treatment effect (LATE). This LATE parameter is identified with a homogeneity assumption as in Section 3. 

%This LATE parameter is related to the indirect effect of $T$ through $D$ in mediation analysis. \cite{HuberSchelkerStrittmatter2019} show point-identifications of a variety of other parameters including the direct and the indirect effects of the compliers using the rank similarity approach. 



==> thesis_Identification.tex <==
\section{Identification}

In this section, I consider the identification assumptions for the ITTTA and ITTNA illustrated through one-sided noncompliance designs.

\subsection{Identification assumption}
%To begin with, we need to note that (\ref{eq.ITTTA}) the ITTTA and
%(\ref{eq.ITTNA}) the ITTNA defined in the previous section are
%well-defined.

If an individualistic assignment causes a direct effect by altering the behavior of units, then the potential outcomes, trivially defined as stable unit treatment value assumption (SUTVA) \citep{Rubin80}, can be justified. If there are spillover or equilibrium effects from community-level interventions, then SUTVA may be violated for the individual observation units. To accommodate the direct effects stemming from strategic interactions, as equilibrium behavior in taking up a treatment, I weaken SUTVA to create unique equilibrium potential outcomes that may depend on community $c$ to which unit $i$ belongs.
\begin{assumption}\label{ass:WDP}
 Let $c$ be a set of observations
 $\{1,\ldots,n_c\}$, with common assignment $T_c \in \{0,1\}$. For every $c, i \in c$, and $t \in \{0,1\}$, there are unique maps for a treatment indicator $D_{i;c}(t)$ and potential outcomes $Y_{i;c}(t,d)$ with
 the corresponding $d$ values in support of $D_{i;c}(t)$. 
\end{assumption}

%\begin{proposition}[Well-defined parameters]
% Let $C$ be a probability space $(C,\Omega,P)$ with each community $c$
% consists of a set of index $\{1,\ldots, n_c\}$ representing
% observations $i$ in the community $c$.
%
% Under the assumption \ref{ass:WDP}, the expectation
% \[
%  P[\frac{1}{n_c} \sum_{i=1}^{n_c} Y_{1,D(i;c)}(i;c) - Y_{0,D(i;c)}(i;c)]
% \]
%\end{proposition}

Throughout this study, I assume that a random sample of units from the population consists of identical
units, representing either individuals or communities. For example, the ITTTA
\[
 E[Y_{i;c}(1,1) - Y_{i;c}(0)|T_c = 1, D_{i;c} = 1]
\]
is the mean comparison of potential outcomes $Y_{i;c}(1,1)$ and $Y_{i';c'}(0)$ from identical
communities $\{c,c'\}$ with $T_c = 1$ against $T_{c'} = 0$ for the same type of members $\{i,i'\}$ who would apply the treatment 
if their communities belonged to the treatment group $T_c = 1$, namely, $D_{i;c}(1) = D_{i';c'}(1) = 1$. Under Assumption \ref{ass:WDP}, the take-up and non-take-up subgroups
are stable and unique for a given draw of communities. 
Nonetheless, I do not observe these take-up or non-take-up members in these communities without assignment $T_c =
0$. Therefore, I need an additional identification restriction. Below,
I omit the index $\{i;c\}$ from the potential outcomes to simplify the notations.
%Therefore, the ITTTA
%is a valid comparison of subgroup members of the treated community $T_c =
%1$ taking the treatment $D_{i;c} = 1$ against the same type of members from an identical
%community without the assignment $T_c = 0$. 

%The primary goal of this paper is to provide an identification strategy
%with endogenous post-treatment covariates $D$ without relying on
%instruments or specific experimental designs. The key idea is the use of an additional
%variable $Y_b$ from a baseline survey as a proxy for the control outcome $Y_0$.
%The baseline survey is data collected before the intervention starts.
%Collecting a baseline survey is a common practice primarily for attaining more precise estimates or studying the subgroup effects with the baseline covariates $W$.

Hereafter, I consider RCTs with the two consecutive surveys of
baseline and intervention. Let $Y_b$ denote a variable observed in the
baseline survey to ensure that $Y_b$ works as a proxy for the control
outcome of interest $Y(0)$. Let $W$ denote a vector of other pretreatment covariates
observed in the baseline survey. I assume that the random assignment of $T$ is
successful for the potential outcomes $Y(0)$ and $Y(1)$ and the baseline
variable $Y_b$.
\begin{assumption} \label{ass:CIZ}
 \[
  (Y(t),D(t)) \indep T | W, \forall t \in \{0,1\},
 \]
 and 
 \[
  (Y_b,D(t)) \indep T | W.
 \]
\end{assumption}

This randomization assumption is sufficient to identify the following ITT
\begin{lemma} \label{lmm:cATE}
 If Assumptions \ref{ass:WDP} and \ref{ass:CIZ} hold, then
 \[
  E[Y(1) - Y(0) | W = w] = E[Y | T = 1, W = w] - E[Y | T = 0,W = w]
 \]
 for every $w \in \mathcal{W}$. 
\end{lemma}
\begin{remark}
Assumption \ref{ass:CIZ} is stronger than necessary for the ITT in the independence of $Y_b$ from $T$. I label this assumption as random assignment because of the restriction on $Y_b$, notwithstanding its similarity to the conditional ignorability for observational data (see Remark 2 for the role of covariates $W$).
\end{remark}

My identification strategy is to exploit certain similarities in the proxy variable
$Y_b$ and control outcome $Y(0)$. However, these two random variables, $Y_b$
and $Y(0)$, may have different distribution functions. Thus, I
restrict the rankings of $Y_b$
and $Y(0)$ to ensure that they are similar. Throughout the study, $F_{Y|W}(\cdot|w)$ represents the conditional
distribution function of the random variable $Y$, and $Q_{Y|W}(\cdot|w)$ constitutes the conditional quantile function of $Y$.
\begin{definition} \label{def:latentRank}
 $W$ is a vector of baseline covariates and random variable $U_w \sim U[0,1]$, indexed by each $W = w$, is termed
 a (conditional) latent rank variable for random variable $Y$ if 
 \[
  Y = Q_{Y|W}(U_W|W)
 \]
 where $Q_{Y|W}(u|w) = \inf\{y: F_{Y|W}(y|w) \leq u\}$ and $u \in [0,1]$.
\end{definition}
The above definition is a key departure from other rank imputation strategies. Many approaches, including \citeauthor{AtheyImbens06}' (\citeyear{AtheyImbens06}) and \citeauthor{HuberSchelkerStrittmatter2019}'s (\citeyear{HuberSchelkerStrittmatter2019}), have assumed that a structural model shares the same scalar latent rank across potential outcomes. Such a structural assumption possibly imposes an obscure restriction on the nature of the random variable, especially when the outcomes are not continuously distributed. On the one hand, it is difficult to avoid such an additional structure function with a common latent variable across outcomes without randomization, as in Assumption \ref{ass:CIZ}. This is because there is no other way to convey the control outcome information from the no intervention units to the intervention units. On the other hand, the structure itself is more than necessary to identify the principal stratification effects when the groups are randomized. I do not assume that such a common latent rank exists across potential outcomes rather that latent rank variable $U_w$ exists for each potential outcome and is a definition as opposed to an assumption. Such a variable exists whether $Y$ is finitely supported or continuous. In fact, we can always construct such a conditional latent variable $U_w$.
%These structures may be natural when the outcome and the proxy variables are repeated measures. Otherwise, these structures are not necessarily reasonable.
Let, $F_{Y|W=w}(y-) \equiv \lim_{\tilde{y} \downarrow y}F_{Y|W=w}(\tilde{y})$, for the right-continuous conditional cumulative distribution function. Moreover,
 \[
  U_w = F_{Y|W}(Y-|w) + V \cdot (F_{Y|W}(Y|w) - F_{Y|W}(Y-|w))
 \]
 where $V \sim U[0,1]$ and $V \indep (Y,W)$, resulting in a quantile function $Q_{Y|W}(\cdot|w)$ that generates the random variable $Y$ (see \citeauthor{Ruschendorf2009}'s (\citeyear{Ruschendorf2009}) Proposition 2.1 for the presence of such a latent variable).

%My identification strategy proceeds in the following three steps. First,
%we construct the observation of $W$-conditional latent ranking of the proxy variable $Y_b$, $U_{b,w}$,
%as the percentile for each observation of $Y_{b,w}$ within the subgroup
%taking the endogenous treatment take-up $D = d$ in the treatment
%group $T = 1$. Second, I assume rank similarity, in other words, the
%distribution of $U_{b,w}$ conditional on $\{D =
%d, T = 1\}$ is the same as the distribution of $U_{0,w}$ conditional on $\{D =
%d, T = 1\}$. Note the event of $Y_0$ less than or equal to $y_0$
%conditional on $W$ has the same
%probability as the event of $U_{0,w}$ less than or equal to
%$F_{Y_0|W}(y_0|w)$ conditional on $W$.%
% represents the value of the
%latent rank of $Y_0$, $U_{0,w}$, at $Y_0 = y_0$ as the fraction 
%$F_{Y_0|W}(y_0|w)$ By rank similarity, 
%the latent rank of $Y_0$ at $y_0$,
%, follows the distribution of $U_{b,w}$ conditional on $\{D =
%d, T = 1\}$. Finally, we can obtain the distribution of $Y_0$ conditional on $\{D =
%d, T = 1\}$ as the fraction of $U_{b,w}$ less than the ranking
%$F_{Y_0|W}(y_0|w)$ conditional on $\{D = d, T = 1\}$.

For the identification, I impose two restrictions on the relationship between
the proxy variable $Y_b$ and the control outcome $Y(0)$. First, I need to
determine the complete latent ranking of $Y_b$, $U_{b,w}$, over the entire support of
$[0,1]$. To achieve the requirement, I assume $Y_b$ has a
strictly increasing and continuous distribution
function.
\begin{assumption} \label{ass:UQ}
$\mathcal{W}$ is the support of $W$, and for every $w \in \mathcal{W}$, $F_{Y_b|W}(\cdot|w)$ is strictly increasing and continuous. %\footnote{This
% condition is equivalent to the conditional quantile function satisfies
%$Q_{Y|W}^b(F_{Y|W}^b(y|w)|w) = y$ for every value of $y$ on the support
% of $Y_b$ conditional on $W = w$.} 
\end{assumption}

This assumption is required to point identify the parameter of interest. Although a partial identification is possible with a finitely supported proxy variable $Y_b$, this is beyond the scope of this study, as my primary focus is point identification. 

Second, I assume that the latent rankings of $Y_b$ and $Y(0)$ are similarly associated with (endogenous) treatment $D$ given $T = 1$. The latent rankings of the same correlation with D is an example of when following rank similarity restriction holds. %However, the reverse condition is not guaranteed.
%This assumption is required for the point-identification of the
%parameter of interest. A partial-identification can be possible with a
%finitely supported proxy variable $Y_b$, but I do not discuss in this
% paper as the primary focus of this paper is to the
% point-identification.
%For the point-identification, I rely on a continuous proxy variable
%$Y_b$. Another key departure from the other CiC approaches is that I do not restrict the potential outcomes $Y(1)$
%and $Y(0)$ being continuously distributed repeated outcome measures of the same
%kinds. These outcomes of interest may be finitely supported for the
%point-identification.
%Second, I assume that the latent rankings of $Y_b$ and $Y(0)$ are similarly associated with the (endogenous) treatment $D$ given $T = %1$ such as the same correlation with $D$:
%assume the latent ranking of $Y_b$ has the same distribution
%as the latent ranking of $Y(0)$ conditional on $W = w,T = 1$ and $D = d$ for $d \in \{0,1\}$, called the rank similarity:
\begin{assumption} \label{ass:RS}
 $U_{b,w}$ is the latent ranking of $Y_b$ and $U_{0,w}$ is the
 latent ranking of $Y(0)$, as defined in Definition \ref{def:latentRank}. %Assume that
 \[
  U_{b,w} \sim U_{0,w} |W = w, T = 1,D = d
 \] 
 for each $d \in \{0,1\}, w \in \mathcal{W}_1$, where $\mathcal{W}_1$ is
 the support of $W$ conditional on $T = 1$.
\end{assumption}
\begin{remark}
The distributions of $Y_b$ and $Y(0)$ may differ arbitrarily, and $Y(1)$ and $Y(0)$ may be finitely supported for point identification. In Appendix C.6, I demonstrate that a binary $Y(0)$ may satisfy both Assumption \ref{ass:UQ} and \ref{ass:RS} with a continuous proxy $Y_b$.

%In the application in Section 5, I analyze a truncated $Y$ using a continuous part of the repeated $Y_b$ at a cost of discarding observations.

The repeated measure of $Y(0)$ in the baseline, namely $Y_b(0)$, is not always available. The discreteness of $Y(0)$ further motivates the use of a nonrepeated $Y_b$ because DiD may predict $Y(0)$ outside the allowable range.
A $Y_b$ that solely determines $Y_b(0)$ given $W$ is a good proxy because the latent rank of $Y_b$ equals that of $Y_b(0)$, which can be identically distributed with the latent rank of $Y(0)$.
As another example of a structure to determine a good proxy, an underlying unobserved determinant $U$, in addition to identical shocks ($\tilde{U}_b, \tilde{U}_0$) called \textit{slippages}, can determine both $Y_b$ and $Y(0)$ (\citealp{HeckmanSmithClements97}). In both cases, conditioning on $W$ affecting $Y(0)$ and $Y_b$ may eliminate multidimensional relations that may violate Assumption \ref{ass:RS}. Appendix C.4 displays the conditions sufficient for Assumption \ref{ass:RS} using structural models with illustrations for the microcredit example (Example C.1).

Note that the rank similarity restriction is on the reduced-form latent ranks. Structural modeling on the latent ranks helps us in justifying the restriction, but the model is not necessary. Randomization helps us in proceeding with reduced-form latent ranks because $(Y(0),Y_b(0))$ are common across treatment and control groups. %If the randomization is absent, then it is difficult to avoid a structural model connecting outcomes in different groups.
\end{remark}
In addition, I assume the following restriction for the support of the covariates $W$:
\begin{assumption} \label{ass:overlapSpp}
$\mathcal{W}_1$ is the support of $W$ conditional that $T = 1$, and
$\mathcal{W}_0$ is the support of $W$ conditional that $T = 0$. Assume that
 $\mathcal{W}_1 = \mathcal{W}_0 \equiv \mathcal{W}$.
\end{assumption} 
\begin{remark}
This assumption imposes a restriction on the population supports, and for the purpose of identification, one can justify Assumption \ref{ass:overlapSpp} with RCT data. %In practice, finite sample failure for this assumption is a challenge for estimating the identified parameter; however, in Section 4, I introduce a semiparametric estimator that should ease this challenge. Moreover, in Appendix E.2, I demonstrate its finite sample performance relative to the parametric implementation proposed by \cite{AtheyImbens06}.
\end{remark}

\subsection{Identification result}
Given the above restrictions, I present the main result. The target parameter is the distribution
$F_{Y(0)|T,D}(y|1,d)$, its quantile, and the mean computed from the
distribution.
\begin{theorem} \label{thm:IdRS}
 If Assumptions \ref{ass:WDP}, \ref{ass:CIZ}, \ref{ass:UQ}, \ref{ass:RS}, and
 \ref{ass:overlapSpp} hold, then
 \[
  F_{Y(0)|W,T,D}(y|w,1,d) =
 F_{Y_b|W,T,D}(Q_{Y_b|W,T}(\tau_{y,w}|w,1)|w,1,d), \tau_{y,w} \equiv F_{Y(0)|W,T}(y|w,0)
 \]
 for every $d \in \{0,1\}, w \in \mathcal{W}$ and $y$ in the support of $Y(0)|W=w,D=d$.
 \begin{comment}
Therefore, 
 \[
  E[Y_{1}|T=1,D=d] - E[Y_0|T=1,D=d]
 \]
 as well as the subgroup quantile difference is identified as
 \[
  Q_{Y|T,D}^1(\tau|1,d) - Q_{Y|T,D}^0(\tau|1,d)
 \]
 for each $d \in \{0,1\}$ where
 \[
  E[Y_0|T=1,D=d] = \int y dF_{Y|T,D}^0(y|1,d),
 \]
 \[
  F_{Y|T,D}^0(y|1,d) = \int F_{Y|W,T,D}^0(y|w,1,d) dF_{W|T,D}(w|1,d),
 \] 
 and
 \[
  Q_{Y|T,D}^t(\tau|1,d) = \inf\{y \in \mathcal{Y}^t :
  F_{Y|T,D}^t(y|1,d) \geq \tau\}
 \]
 for every $\tau \in [0,1]$ and each $t \in \{0,1\}$.
\end{comment}
\end{theorem}
\begin{proof}
 See Appendix B.
\end{proof}

\begin{center}
  \begin{figure}[h!]
  %\includegraphics[width=0.95\textwidth]{FormulaAltPaper.eps}
   \includegraphics{FormulaAltPaper2.eps}
 \caption{A graphical representation of the identification formula. In
   both panels, the $x$ axis shows the level of the outcome measures $Y(0)$ and
   $Y_b$, and the $y$ axis represents the level of the latent rank variables $U_0$ and
   $U_b$. Panel A offers the map from $y_0$ in the support of $Y(0)$
   into $F_{Y(0)}(y_0)$ in the support of $U_0$. Panel B
   presents the map from $F_{Y(0)}(y_0)$ in the support of $U_b$ into
   $Q_{Y_b}(F_{Y(0)}(y_0))$ in the support of $Y_b$.}
  \label{fig:Formula}
  \end{figure} 
\end{center}

Figure \ref{fig:Formula} summarizes the concept underlying the formula. For simplicity, we can consider the case without the covariates W. As Panel A in Figure \ref{fig:Formula} describes, the events $\{Y(0) \leq y\}$ and $\{U_0 \leq F_{Y(0)}(y_0)\}$ are equivalent almost surely for every $y_0$ in the support of $Y(0)$, $\mathcal{Y}_0$. Although $Y(0)$
may have a positive mass in the support of $Y(0)$, it does not hamper this step because we only need to evaluate $F_{Y(0)}(y_0)$ in the support of $Y(0)$. Rank
similarity equates the events of $\{U_0 \leq F_{Y(0)}(y_0)\}$ and $\{U_b
\leq F_{Y(0)}(y_0)\}$, with a conditional expectation of $\{T = 1, D =
d\}$. As Panel B in Figure \ref{fig:Formula} shows, we may find the quantile of
$Y_b$ in the support of the random variable $U_b$. Such a quantile
$Q_{Y_b}(u)$ can be found for every $u \in [0,1]$ from the continuity of
$Y_b$. Therefore, for every value of the latent rank $F_{Y(0)}(y_0)$, we
can indicate its quantile $Q_{Y_b}(F_{Y(0)}(y_0))$ in terms of $Y_b$. Then the events $\{U_b \leq
F_{Y(0)}(y_0)\}$ and $\{Y_b \leq Q_{Y_b}(F_{Y(0)}(y_0))\}$ have the same
probability conditional on $\{T = 1, D = d\}$. Thus, I equate the conditional expectation of $\{Y(0) \leq y\}$
with that of $\{Y_b \leq Q_{Y_b}(F_{Y(0)}(y_0))\}$. 

While standard CiC approaches (\citealp{AtheyImbens06}; \citealp{HuberSchelkerStrittmatter2019}) include a support condition for the latent rank variable, this condition is not presented in this study because I do not impose a structural function with a common latent rank variable across the functions. I define the latent ranks from the potential outcome as uniform random variables on $[0,1]$, and impose a direct pairwise relation in unobserved ranking variables $U_{0,w}$ and $U_{b,w}$. This direct relation is a distinction from the control function approaches (e.g., \citealp{ImbensNewey2009};
\citealp{DHaultfoeuilleFevrier2015}; \citealp{Torgovitsky2015};
\citealp{Ishihara2017})
 
%Therefore, I do
% not require an excluded instrument to recover the relation in the two
% unobservables, unlike it is the case for the control function approach.

\subsection{ATT identification with homogeneity restriction}

With the rank similarity binding the control outcome and proxy variable, I present the ITTTA and ITTNA identification process without, for example, imposing restrictions on $Y(1,0)$ and $Y(1,1)$. Although the ITTTA and ITTNA have important scientific and policy implications, I may be able to separate the ATT from the ITTTA if the following homogeneity assumption holds.
\[
 E[Y(1,0) - Y(0)|T = 1, D = 1] = E[Y(1,0) - Y(0)|T = 1, D = 0]. 
\]
%\begin{assumption}[Homogeneity of direct effect for one-sided noncompliance]
% \[
% 
% \]
%\end{assumption}
The above assumption indicates that the direct effect $Y(1,0)-Y(0)$ has the same mean for the treated and nontreated. This homogeneity assumption is related to the exclusion restriction, $E[Y(1,0) - Y(0)|T = 1, D = 1] = 0$, and is substantially weaker. One can consider the exclusion restriction as a special case, as the homogeneous direct effect is 0. With the homogeneity, the ATT, $E[Y(1,1) - Y(1,0)|T = 1, D = 1]$, is simply the difference between the ITTTA and ITTNA, $E[Y(1,1) - Y(0)|T = 1, D=1]-E[Y(1,0) - Y(0)|T = 1, D = 0]$.
This homogeneity restriction may be justified when the assignment effect is universal across units. For example, if the assignment causes an equilibrium effect on the local prices of essentials, then the homogeneity assumption may hold. By contrast, if the assignment causes a spillover effect that affects the treated and nontreated differently, then the assumption is implausible. Although this restriction is strong, I have two justifications for the above quantity. First, it is challenging to separate the ATT from the ITTTA unless scalar unobservable restrictions are imposed on both $Y(1,0)$ and $Y(1,1)$. Second, the above quantity may still operate as a back-of-the-envelope calculation of the magnitude of the ATT. For example, as the spillover of microcredit access may represent a transfer from the treated to the nontreated, the direct effect for the treated may be lower than that of the nontreated. In that case, the ATT value may be underestimated with the back-of-envelope calculation (see Section 5 for its application to the microcredit experiment and Section 6 for the complexities of this concept for two-sided cases).

%I admit that this restriction is strong. Nevertheless, I have two justifications for the above quantity. First, it is challenging to separate the ATT from the ITTTA unless we are willing to impose scalar unobservable restrictions also on $Y(1,0)$ and $Y(1,1)$. Second, the above quantity may still work as a back-of-envelope calculation for the magnitude of the ATT. For example, the spill-over of microcredit access may be a transfer from the treated to the nontreated, and therefore, the direct effect for the treated may be smaller than the direct effect for the nontreated. In that case, it gives a possibly underestimated value of the ATT. See Section 5 for its application to the microcredit experiment. In Section 6, I explore a complication in this concept for the two-sided cases.

%Note that this homogeneity assumption is a related concept of so called additivity or no interaction effect as in \cite{Holland_1988} or \cite{Robins_2003} (cf. \citealp{Imai_Tingley_Yamamoto_2013}) in particular when the concept is extended to the two-sided noncompliance case. See Section 6 for the discussion.

%[No this is for the two-sided case]This homogeneity assumption is a weaker concept of so called additivity or no interaction effect as in \cite{Holland_1988} or \cite{Robins_2003} (cf. \citealp{Imai_Tingley_Yamamoto_2013}), requiring only the mean of direct effects equal but not the 


==> thesis_Introduction.tex <==
\section{Introduction}
Randomized assignment is a standard strategy to identify the average treatment effect under full compliance (i.e., when the assignment equals the associated treatment). By contrast, under noncompliance, an additional exclusion restriction is required to identify the associated treatment effects. Although an exclusion restriction requires that the assignment has no causal effect on the outcomes holding the treatment status fixed, this restriction may not always hold. In fact, the assignment itself may affect the outcomes for several reasons. 

%The ITT is usually not the
%primary parameter of interest. The ITT is not the effect of the
%treatment, as not everyone takes the treatment. Instead, the ITT is the
%effect of the assignment. It is a weighted mean of
%heterogeneous treatment effects by the treatment take-up behavior. The
%other parameter of interest in which
%we are frequently interested is the treatment effect for those who take
%up the treatment, called the
%average treatment effect on the treated (ATT). The ITT identifies the
%effect of treatment assignment whereas the ATT reveals the effect of
%taking the treatment for the subgroup of the treated. However, the ATT
%is not
%identified simply by randomization of treatment assignment.

For randomized control trials (RCTs), I propose a strategy to identify the effects of a binary assignment and binary treatment without imposing an exclusion restriction. Specifically, I consider the intention-to-treat (ITT) effects decomposed by the treatment status. There are two key parameters to consider. First, I consider the ITT conditional on the treated under the assignment (ITTTA). The ITTTA is the combined effect of both the assignment and the treatment. It equals the average treatment effect on the treated (ATT), when the exclusion restriction holds under one-sided noncompliance, which prohibits the units from taking up the treatment without the assignment. Second, I consider the ITT conditional on the nontreated under the assignment (ITTNA). The ITTNA is solely the assignment's own effect, often referred to as the assignment's direct effect.

To identify the heterogeneous effects of whether to employ the treatment, the baseline strategies are to either use the assignment as an instrumental variable (IV) or the conditionally ignorable assumption for the treatment. In my strategy, I require neither the exogenous treatment nor valid IVs. Instead, I develop a natural experimental approach in RCTs with their typical feature, that is, the baseline survey. I use a continuous variable from the baseline survey as a proxy for the control outcome. Specifically, I develop a rank imputation strategy with new estimators based on a rank similarity assumption that appears in \citeauthor{ChernozhukovHansen05}'s (\citeyear{ChernozhukovHansen05}) quantile IV model as well as in \citeauthor{AtheyImbens06}'s (\citeyear{AtheyImbens06}) change-in-changes (CiC) model. I apply the method to microcredit and cash transfer experimental studies and demonstrate that the direct effect of the randomized assignment for the nontreated, the ITTNA, is an attractive and important parameter for estimating the combined effect of the assignment and the treatment, the ITTTA.

%leading paragraph for the contribution
This study makes three major contributions to the literature. First, I propose a natural experimental strategy for RCTs by exploiting their typical feature, the baseline survey. Specifically, the first contribution concerns the parameter, called principal stratification by \cite{FrangakisRubin2002}, that appears when exploring for the causal effect mechanism. Causal inference with an invalid instrument for the treatment is the leading context in principal stratification. For example, \cite{DeuchertHuber2017}, who examined the Vietnam draft lottery, documented that the exclusion restriction may be violated. Furthermore, most studies in this context exploit exclusion restrictions (\citealp{ImbensAngrist1994}; \citealp{AngristImbensRubin96}) or conditional independence (\citealp{HiranoImbensRubinZhou2000}).

%I have three major contributions. First, I propose a natural experimental strategy for RCTs exploiting their typical feature of the baseline survey. Compared to \cite{HuberSchelkerStrittmatter2019} who consider a richer mediation analysis under richer models and restrictions, the proposed strategy requires fewer model structures and less restrictive assumptions to point-identify the principal strata parameters. Second, I find that the CiC strategy does not necessarily require repeated outcome measures for the point-identification. I demonstrate the CiC strategy with binary or discrete outcomes to point-identify the treatment introduced over time when there is a continuous proxy variable in the baseline. Third, I propose an estimator of the rank imputation strategy. The estimator fixlbely incorporates covariates relative to the existing implementation of \cite{AtheyImbens06}. I demonstrate its desirable finite sample performances in clustered sampling, as well as its robustness to nonlinear mean outcome functions, which invalidate the parametric implementation of \cite{AtheyImbens06}. Below, I detail the three contributions in the literatures.

%Therefore, this paper complements \cite{HuberSchelkerStrittmatter2019} to offer an option to applied researchers to trade-off the strength of the restrictions and the richness of the parameters. 

As an alternative, several studies (\citealp{ZhangRubin2003}; \citealp{Rubin2006}; \citealp{FloresFloresLagunes2013}; \citealp{MealliPacini2013}) have proposed partial identification strategies exploiting monotone treatment response arguments (\citealp{Manski1997}; \citealp{ManskiPepper2000}). In response to the above baseline strategies, the natural experimental approach has also emerged as a substitute recently. For instance, \cite{DeuchertHuberSchelker2018} used a difference-in-differences (DiD) strategy to study the Vietnam war draft's impact on political preferences. Specifically, the analysis allowed for the draft itself to have a direct impact on the preferences. Additionally, \cite{HuberSchelkerStrittmatter2019} proposed a CiC strategy for the principal stratification and mediation analysis to study the impact of job training on mental health, using a randomized job training program in the United States called JOBS II. A unique feature of \cite{HuberSchelkerStrittmatter2019} appears in their results without valid randomization. Specifically, they applied their strategy without valid randomization when examining the effect of paid maternity leave on labor income, using the Swiss Labour Force Survey.

 %However, the DiD approach has two limitations. First, the
%DiD strategy does not identify quantile effects. Second and more importantly, the DiD
%approach requires the exact repeated measures before and after the intervention. The former issue has been resolved by \cite{HuberSchelkerStrittmatter2019}, but they do not deal with the latter issue.
%I contribute to this literature by offering a unique natural experimental strategy which exploits the baseline survey, and the proposed strategy resolves the latter issue of the DiD alternative.

%The proposed strategy differs from \cite{HuberSchelkerStrittmatter2019} in a number of reasons described below.
%My rank imputation strategy exploits a continuous proxy variable in the baseline survey. 
Thus, I contribute to this stream of the literature by offering a unique natural experimental strategy that exploits the baseline survey with a continuous proxy variable. I impose restrictions on the proxy variable and the control outcome in their latent rankings, which are uniform random variables representing their underlying percentiles. I assume that the conditional distributions of the latent rankings for the proxy variable and control outcome are identical regardless of whether taking up a treatment. This restriction is called the rank similarity assumption, under which taking up a treatment may be endogenous. Although the strategy is consistent with \cite{HuberSchelkerStrittmatter2019}, my aims and imposed restrictions differ in two ways. First, \cite{HuberSchelkerStrittmatter2019} required a structural model with a common latent rank variable unifying the different potential outcomes. Although the functional form is entirely flexible, it is a strong restriction in which a single unobserved variable governs all the potential outcome values during the same period. As I define the latent ranks as reduced-form representations for each potential outcome, I do not impose the structural model or the common latent rank variable. Second, to fully uncover the parameters, \cite{HuberSchelkerStrittmatter2019} imposed latent rank restrictions not only on the control outcomes against the proxy but also on the treatment outcomes against the proxy. While the proxy variable and control outcome, which are both free of the intervention, are similar, it is challenging to relate the treatment outcomes to the proxy in general. Nonetheless, these stronger restrictions allow them to identify the mediation effects and principal stratification without randomization. Furthermore, it is difficult to disentangle the restrictions on the control and treatment outcomes because both are unified in the common latent rank, and the restrictions are imposed on the common latent rank variable. In my strategy, I do not impose any restrictions on the treated outcome, given the potential outcome model under randomization for the ITTTA and ITTNA. Instead, I only impose restrictions on the control outcomes. As these weaker restrictions prohibit us from identifying the other parameters in \cite{HuberSchelkerStrittmatter2019}, I impose fewer necessary restrictions on the potential outcomes to identify the parameters relating to the principal strata. 

Overall, compared with \cite{HuberSchelkerStrittmatter2019}, who considered a richer mediation analysis under richer models and restrictions, the proposed strategy requires fewer model structures and less restrictive assumptions to identify the principal strata parameters. Therefore, this study complements \cite{HuberSchelkerStrittmatter2019} by offering another option for applied researchers to trade off the strength of the restrictions and richness of the parameters. In general, one can use my strategy for minimal key parameters and \citeauthor{HuberSchelkerStrittmatter2019}'s (\citeyear{HuberSchelkerStrittmatter2019}) if stronger restrictions are justified to study the causal effect mechanisms in depth.

% These distictions appear in the main analysis of one-sided noncompliance, but it becomes sharper in the case of two-sided noncompliance. See further discussions in Section 3 and 6.

% I resolve the limitation in the earlier natural experimental approaches such as \cite{DeuchertHuberSchelker2018} and \cite{HuberSchelkerStrittmatter2019} which consider exact reapted outcome measures before and after the intervention. This feature is also a general contribution to rank imputation strategies. 

As a second contribution, I find that the CiC strategy does not necessarily require repeated outcome measures for point identification. I demonstrate that the CiC strategy with binary or discrete outcomes can be used to identify the treatment effect when there is a continuous proxy variable in the baseline. My approach again differs from \cite{HuberSchelkerStrittmatter2019}, who considered an identification with continuous repeated outcomes. Many rank imputation approaches involve rank similarity or a stronger version, rank invariance (\citealp{JuhnMurphyBrooks93}; \citealp{DiNardoFortinLemiux96}; \citealp{AltonjiBlank99}; \citealp{ChernozhukovHansen05}; \citealp{MachadoMata05}). An alternative copula restriction also reveals the identification of the conditional quantile treatment effects (\citealt{CallawayLiOka17}), but the rank similarity approach is dominant. More recently, \cite{Han2018} used the rank similarity assumption to identify dynamic treatment effects with nonseparable models and \cite{deChaisemartinDHaultfoeuille2017} studied the fuzzy design of CiC models under the assumption of an exclusion restriction.

Among these rank similarity-based approaches,  \citeauthor{AtheyImbens06}' (\citeyear{AtheyImbens06}) CiC strategy is a natural experimental approach. As a generalization of the DiD model, a CiC strategy considers repeated outcome measures. For example, the underlying motivation in \citeauthor{AtheyImbens06}' (\citeyear{AtheyImbens06}) CiC strategy was to examine the issue in the standard DiD model, specifically because discrete outcomes may be predicted outside their supports. However, a CiC strategy with discrete repeated outcomes does not identify the parameters without stronger restrictions. Thus, I demonstrate that a CiC strategy may work without repeated outcomes. Specifically, I reveal the process of identifying the parameters of interest with discrete outcomes predicted from a continuous proxy variable. The key observation is that I do not need to invert the distribution function of the control outcome, allowing for a discrete outcome measure for point identification. Random assignment helps to justify this strategy. Particularly, randomization creates symmetry in the control outcome and proxy variable distributions across the units with and without the intervention. This symmetry allows us to directly compare the potential outcomes observed for units without an intervention versus units with an intervention, rather than going through the unifying structural functions. One can seek a proxy variable that is not necessarily the exact repeated measure because the structural function with the common latent rank in RCTs does not serve any essential role. This finding is particularly important in the context of RCTs because repeated measures may be unavailable. For example, an outcome such as timely graduation from a school cannot be repeated; conversely, the administrative records of test scores may be applicable as the graduation proxy. In this example, while the DiD does not apply, the rank imputation strategy may allow us to identify the assignment and treatment effects.

As the third contribution, I propose an estimator of the rank imputation strategy that is valid for any type of outcome measure and can flexibly incorporate covariates that have been compared with \citeauthor{AtheyImbens06}' (\citeyear{AtheyImbens06}) implementation. I demonstrate its desirable finite sample performance in clustered sampling as well as its robustness to nonlinear mean outcome functions that invalidate \citeauthor{AtheyImbens06}' (\citeyear{AtheyImbens06}) parametric implementation. Specifically, \cite{AtheyImbens06} proposed a nonparametric estimator with discrete covariates, but the implementation with continuous covariates took a restrictive parametric form. Similarly, \cite{MellySantanglo15} suggested a semiparametric estimator with covariates, in response to the general theory used by \cite{ChernozhukovFernandezValMelly13}; however, the strategy is less appealing for a CiC model without quantile functions of repeated outcome measures. Alternatively, I propose another semiparametric estimator based on distribution regressions. In Appendices A.1 and A.2, I discuss the weak convergence of the empirical process for the proposed counterfactual estimator and the validity of the bootstrap inferences. I also adopt \citeauthor{DaveziesDHaultfoeuilleGuyonvarch18}'s (\citeyear{DaveziesDHaultfoeuilleGuyonvarch18}) results of cluster-robust weak convergence to accommodate the experimental studies with cluster dependencies. I demonstrate the estimators' finite sample performance in simulations in Appendix E.1 and compared this with \citeauthor{AtheyImbens06}' (\citeyear{AtheyImbens06}) incorporation of covariates in Appendix E.2.

%\footnote{There are advantages and disadvantages of
%quantile regression and distribution regression. While it is
%straightforward to estimate conditional quantile
%functions in quantile
%regression, a tail-trimming procedure is required to estimate the
%conditional distribution functions. For the primary purpose of the mean
%effect unconditional of the covariates, it is necessary to obtain the
%conditional
%distribution functions for the full support of the outcome of interest.}
I apply the proposed estimator in the context of an experimental approach in development economics. In particular, I use the data from \cite{CreponDevotoDufloPariente2015}, who conducted a large-scale microcredit experiment in Morocco, to estimate the ITTTA, representing the intervention's combined effects. In addition, I separately estimate the ITTNA, which is the direct effect of the assignment for the nontreated, finding that the corresponding IV point estimate is 2.2 times larger than my preferred ITTTA estimate. Nevertheless, the estimated effects are not statistically different because of the large standard errors. The signs and magnitudes of the suggested ITTTA and ITTNA estimates may imply the possibility of a small, but positive direct assignment effect, while the treatment itself should have a large positive impact. As a result, I demonstrate that the small direct effect may be heavily biased in the ATT's IV point estimate, which should equal the ITTTA under the exclusion restriction. I also apply my strategy to \citeauthor{Gertler_Martinez_Rubio-Codina_2012}'s (\citeyear{Gertler_Martinez_Rubio-Codina_2012}) two-sided noncompliance experiment that studied the long-term impact of a cash transfer policy in Mexico. In particular, I evaluate their claim that the assignment's long-term effect is mainly caused by productive animal investments (See Appendix F for the description of the latter's application).

%Development economists are
%interested in the effect of expanding access
%to microcredit opportunities in developing
%countries. See \cite{BanerjeeKarlanZinman2015} for a summary of six recent
%experiments in different locations. For example, \cite{AngelucciKarlanZinman15} and
%\cite{CreponDevotoDufloPariente2015} run large-scale microcredit
%experiments in Mexico and Morocco. In these experiments, microcredit companies visit treatment villages, and these
%companies provide microfinance opportunities. Despite new credit being
%available, not all people in treated villages borrow from the
%microcredit firms. These studies aim to evaluate the effects of the treatment, which is the loan from the microcredit firms. However,
%the conventional IV strategy might be invalid because the assignment, which is the randomized access to microcredit, might have a direct effect on business outcomes of
%interest. In fact, there are a number of reasons why this direct effect may occur.

%For
%example, the availability of credit may change the behavior of the
%subjects, including those who would not ex-post use the credit. The
%experimental randomization at the village level may generate a direct
%effect of access. For example, the local village economy might be altered
%by the equilibrium effect through the interest rate of informal lending
%or local sales price changes. Transfers among relatives or friends
%generate positive or negative spillover to those who do not borrow
%credit.
 %I point out that the IV estimate of the ATT, which is consistent
%under the assumption of no direct effect, is subject to bias if the
%direct effect is nonzero. The bias can be enormous even for a small
%direct effect when the take-up rate is relatively low.

%Among many studies of microcredit experiments,
%\cite{CreponDevotoDufloPariente2015} collect a detailed baseline
%survey. 

%\footnote{\cite{CreponDevotoDufloPariente2015} construct subgroups
%with predicted borrowing probabilities. People with predicted
%probabilities of borrowing lower than 30\% are considered
%nonborrowers. Knowing that there is no effect on those
%nonborrowers, the authors conclude that there is no evidence of
%externality. For the discussion of their approach, see the application
%of section 5.}
%As decisions
%to implement a policy relies on the point estimates of the
%heterogeneity
%in the treatment effects, the quantified magnitude of the bias is
%important for
%policy evaluation.

The rest of this paper is organized as follows. Section 2 introduces the notations and parameters of interest, Section 3 lists the formal identification assumptions illustrated in cases of one-sided noncompliance, and Section 4 demonstrates the estimation procedure with uniformly valid and cluster-robust bootstrap inferences. I apply the procedure to an experimental microcredit study in Section 5, discuss the framework in the case of two-sided noncompliance models in Section 6, and present my conclusions in Section 7.

==> thesis_Parameter.tex <==
\section{Parameters of interest}

Consider a standard model of potential outcomes. Let $T \in \{0,1\}$ be a binary randomized assignment and $Y$ be an observed outcome generated out of the potential outcomes. Assignment $T$ indexes the potential outcomes $Y(1)$ and $Y(0)$, such that $Y = T Y(1) + (1 - T)Y(0)$. Assignment $T$'s average effect
\[
 E[Y(1) - Y(0)] = E[Y(1)] - E[Y(0)],
\]
is the ITT. The ITT involves any assignment effects, including the associated treatment effect that assignment $T$ enables or enhances. Although this unconditional ITT represents assignment $T$'s average effect, a study's eventual goal often regards the associated treatment rather than the assignment.

Assume that the binary assignment of $T$ introduces another binary treatment $D \in \{0,1\}$. The units, which are the experimental subjects, choose $D$ endogenously after assignment $T$. If a unit is assigned to the control group ($T = 0$), then the treatment is not available ($D = 0$). The units with assignment $T = 1$ may not comply with the associated treatment $D$. Therefore, $D$ may be either $0$ or $1$ if the unit is in the treatment group $T = 1$.
\begin{definition}\label{def:onesided}
 A design $(Y,D,T)$ satisfies the one-sided noncompliance if 
 \[
  D = 
  \begin{cases}
   0 \mbox{ or } 1 & \mbox{ if } T = 1\\
   0  & \mbox{ if } T = 0.
  \end{cases}
 \]
\end{definition}
The following is an example of a one-sided noncompliance experiment.
\begin{example}
Microcredit experiments are an example of investigations in which researchers are aware of and interested in an assignment's direct impact. Specifically, \cite{CreponDevotoDufloPariente2015} studied the effect of introducing microcredit in Morocco's rural areas. They randomly assigned villages into treatment villages $(T = 1)$ and control villages $(T = 0)$, and the microcredit treatment $D$ followed one-sided noncompliance.
\end{example}
With treatment $D$, the observed outcome is 
\[
 Y = TY(1) + (1 - T)Y(0) = T(DY(1,1) + (1 - D)Y(1,0)) + (1 - T)Y(0)
\]
where $Y(1,1)$ is the outcome given the assignment $(T = 1)$ and taking up
the treatment $(D = 1)$; $Y(1,0)$ is the outcome given the assignment
$(T = 1)$, but not taking up the treatment $(D = 0)$; and $Y(0)$ is the outcome of
the control group, with $T = 0$ and $D = 0$. The leading parameter of interest is the
following ITT conditional on $T = 1$ and $D  = 1$,
\begin{equation}
 E[Y(1) - Y(0)|T = 1, D = 1] = E[Y(1,1) - Y(0)|T = 1, D = 1].\label{eq.ITTTA}
\end{equation}
I define the left-hand side of (\ref{eq.ITTTA}) as the ITTTA, where the equality to the right-hand side of (\ref{eq.ITTTA}) holds under Definition \ref{def:onesided}. Specifically, under Definition \ref{def:onesided},
the ITTTA is the combined effect of 
the ATT,
\[
 E[Y(1,1) - Y(1,0)|T = 1, D = 1],
\]
and assignment $T$'s effect on the treated, net of treatment $D$
\[
 E[Y(1,0) - Y(0)|T = 1, D = 1].
\]
The latter parameter is often called the direct effect of the treated in the principal stratification literature (\citealp{HiranoImbensRubinZhou2000}; \citealp{FrangakisRubin2002}; \citealp{FloresFloresLagunes2013}; \citealp{MealliPacini2013}) and mediation analysis literature (\citealp{Pearl14}). Examining if the ITTTA is significant confirms that experimental assignment $T$ operates through the expected channel of treatment $D$ since intention $T$ or treatment $D$ have impacts, at least for the intended units that comply with the intention. As an analogue parameter, I consider 
\begin{equation}
 E[Y(1) - Y(0)|T = 1, D = 0] = E[Y(1,0) - Y(0)|T = 1, D = 0], \label{eq.ITTNA}
\end{equation}
and I define the left-hand side of (\ref{eq.ITTNA}) as the ITTNA, where the equality holds under Definition \ref{def:onesided}. This ITTNA, the direct effect of the nontreated, has an important policy implication because it indicates if assignment $T$ has a direct impact on the outcome without considering the treatment.
The left-hand-side definitions of the ITTTA and ITTNA represent the same parameters of interest for both one-sided and two-sided noncompliance, while their underlying principal strata differ. Nevertheless, the above interpretation remains similar (see Section 6 for details). The distinction appears when we are interested in separating the net effect of $D$ from the ITTTA and ITTNA (see Section 3.3 for one-sided noncompliance and Section 6.3 for two-sided noncompliance).

%Nevertheless, their interpretation and identification assumptions may differ. See Section 6 for their distinctions. In Section 3, I also discuss an additional assumption to identify the ATT separately from the ITTTA and the ITTNA.

In RCTs, $T$ is randomly assigned, but the treatment
 $D$ may be endogenous. For one-sided noncompliance, running a regression of $Y$ on $T$ and $D$ without covariates may produce a biased estimate in the coefficient of $D$ due to selection bias
\citep{AngristPischke09}. Namely,
\begin{align*}
 E&[Y|T = 1, D = 1] - E[Y|T = 1, D = 0] = E[Y(1,1)|T = 1,D = 1] - E[Y(1,0)|T = 1,D = 0]\\
 =& \underbrace{E[Y(1,1) - Y(1,0)|T = 1,D = 1]}_{\text{the ATT}} 
 + \underbrace{E[Y(1,0)|T=1,D = 1] - E[Y(1,0)|T=1,D = 0]}_{\text{selection bias}}.
\end{align*}

Therefore, researchers often employ random assignment $T$ as the
IV for taking up treatment $D$. Under three
conditions, (i) random assignment $T \indep Y(t)$, (ii) relevancy
$Cov(T,D) \neq 0$, and (iii) the exclusion restriction $E[Y(1,0) - Y(0)|T  = 1, D = 0] = 0$,
the IV estimator identifies the ITTTA, which equals to the ATT,
\begin{align*}
 \frac{Cov(Y,T)}{Cov(T,D)} =& \frac{E[Y(1) - Y(0)]}{P(D=1|T = 1)}\\
=& E[Y(1) - Y(0)|T = 1,D = 1] = E[Y(1,1) - Y(1,0)|T = 1, D = 1].
 %=& E[Y_1 - Y_0|T = 1,D = 1]\frac{P(D = 1|T = 1)}{P(D = 1|T = 1)}\\
 %&+ E[Y_1 - Y_0|T = 1,D = 0]\frac{P(D = 0|T = 1)}{P(D = 1|T = 1)} \\
 %=& E[Y_{11} - Y_0|T = 1,D = 1]\\
 %&+ E[Y_{10} - Y_0|T = 1,D = 0]\frac{P(D = 0|T = 1)}{P(D = 1|T = 1)}\\   %\footnote{Note that
%$\frac{Cov(Y,T)}{Cov(D,T)} = \frac{E[Y_1 - Y_0]P(T=1)P(T=0)}{P(D = 1|T =
% 1)P(T=1)P(T=0)} = \frac{E[Y_1 - Y_0]}{P(D=1|T = 1)}$.}
\end{align*}
where the last equality, based on the exclusion restriction (iii), may not hold. In particular,
assignment $T$ may affect the outcome for those who
do not take up treatment $D$.
\begin{example}%[Example of microcredit experiment, Continued] 
 \cite{CreponDevotoDufloPariente2015} listed several reasons why giving access to assignment $T$ may have an impact even for those who do not borrow $D$ from the microcredit institution:
\begin{quote}
 There are good reasons to believe that microcredit availability
 impacts not only on clients, but also on non-clients through a variety
 of channels: equilibrium effects via changes in wages or in
 competition, impacts on behavior of the mere possibility to borrow in
 the future, etc. (\citealp{CreponDevotoDufloPariente2015}, p. 124)
\end{quote}
 This possibility of the direct impact of availability not only complicates identifying the heterogeneous treatment effects but also emphasizes the importance of the direct impact for understanding the consequences of microcredit intervention.
 %\footnote{\cite{CreponDevotoDufloPariente2015} challenge
 %the estimation of the direct effect based on approach implicitly
 %relying on conditional independence of treatment take-up. For
 %further discussions, see supplementary appendix.}
 %\footnote{Readers may wonder if the possible
 %violation of SUTVA assumption may appear with the spill-over and
 %equilibrium realization of the treatment take-up $D$. In the
 %next section, I demonstrate that the typical modification of
 %considering a village cluster as a unit would work to justify a
 %modified SUTVA assumption.}
\end{example}
If the exclusion restriction is violated, then the IV estimator also becomes a biased ITTTA estimator:
\begin{align*}
 \frac{Cov(Y,T)}{Cov(T,D)} =& E[Y(1) - Y(0)|T = 1,D = 1]\frac{P(D = 1|T = 1)}{P(D = 1|T = 1)} \\
&+ E[Y(1,0) - Y(0)|T=1,D = 0]\frac{P(D = 0|T = 1)}{P(D = 1|T = 1)}.
\end{align*}
The degree of bias depends on the
take-up rate $P(D = 1|T = 1)$. If $P(D = 1|T = 1) > 0.5$, then the
magnitude of the bias is less than $E[Y(1,0) - Y(0)|T  = 1, D = 0]$, but the IV point estimate may have been inflated in absolute value through divisions of the small probability $P(D = 1|T = 1)$ when the take-up rate is low.

Researchers frequently avoid using the IV estimator and report the ITT estimate because of the former issue of bias in the IV estimator. However, the ITT does not reveal the impact that appears because of the treatment in addition to the assignment (i.e., ITTTA), nor the impact appearing solely by the assignment (i.e., ITTNA).

\begin{comment}
 Throughout the paper, $F_{Y(t,d)|W}(\cdot|w)$ represents conditional
distribution function of the random variable $Y(t,d)$ for each $t \in \{0,1\}$ and $d \in \{0,1\}$. Also, $Q_{Y(t,d)|W}(\cdot|w)$ represents conditional
quantile function of the random variable $Y(t,d)$ for each $t \in \{0,1\}$ and $d \in \{0,1\}$.
In the following section, we focus on the case of one-sided noncompliance. Therefore, we propose an identification
strategy for the ITTTA
\[
  E[Y(1,1) - Y(0)|T  = 1, D = 1]
\]
and its quantile differences evaluated at each percentiles $\tau \in [0,1]$
\[
 Q_{Y(1,1)|D,T}(\tau|1,1) - Q_{Y(0)|D,T}(\tau|1,1)
\]
as wel as the direct effect of the assignment for non-treated, the ITTNA
\[
  E[Y(1,0) - Y(0)|T  = 1, D = 0]
\]
and its quantile differences evaluated at each percentiles $\tau \in [0,1]$
\[
 Q_{Y(0,1)|D,T}(\tau|0,1) - Q_{Y(0)|D,T}(\tau|0,1),
\]
exploiting the baseline survey, which is the typical feature of the
randomized control trials. See Section 6 for the parameters and their identifications in two-sided noncompliance cases.
 %\footnote{\cite{AbbringHeckman2007} mention
%that one might be interested in quantiles of $Y_1 -
%Y_0$ rather than the quantile difference in the main text. However, the
%identification of this alternative parameter requires generally harder
%assumptions than the assumptions studied in this paper. Therefore, this
%paper does not study this alternative parameter.}
\end{comment}

\begin{comment}
Replce somewhere 
\subsection{Subgroup effects and mediation effects}

One may wonder why my focus is on the quantity
\[
 E[Y_1 - Y_0|T = 1,d(1,\eta) = d] = E[y(1,d(1,\eta),U) - y(0,d(0,\eta),U)|T = 1,d(1,\eta) = d].
\]

For the evaluation of the treatment $T$ without any further manipulations
available, we need to evaluate the outcome
functions $y(t,\cdot,U)$ at the value of post-treatment variables $D$ as
people choose under their assigned policy $T = t$, i.e.,
$d(t,\eta)$. Therefore, the random variable
\[
 Y_1 - Y_0 = y(1,d(1,\eta),U) - y(0,d(0,\eta),U)
\]
is the relevant treatment effect for every unit $(\eta,U)$. For example,
borrowing decisions and parental investments are not policy variables to
be manipulated by the policy makers in the evaluation or the
implementation of the micro credit treatment and the Head Start
treatment. Thus, the parameters essential for evaluating these treatments are the
overall average effect as the unconditional mean of the above
\[
 E[Y_1 - Y_0] = E[y(1,d(1,\eta),U) - y(0,d(0,\eta),U)]
\]
as well as the subgroup average for those assigned to treatment $T = 1$ and took an
action $d(1,\eta) = d$,
\[
 E[Y_1 - Y_0|T = 1,d(1,\eta) = d] = E[y(1,d(1,\eta),U) - y(0,d(0,\eta),U)|T = 1,d(1,\eta) = d].
\]

We would be interested in far more variety of parameters for different purposes. It is true that obtaining the structural function
\[
 y(t,d,U)
\]
is desirable if we are interested in the causal effect of $d$ on the outcome $y(t,\cdot,U)$ which is by itself an important parameter for understanding the mechanisms behind the treatment effects, or evaluations of a policy with both $D$ and $T$ are manipulable treatments. However, identification of the structural functions require either a presence of a valid instrument (for example,
\citealp{ChernozhukovHansen05}) or an assumption that $D$ is
exogenous to $U$ conditional on $W$ (for example,
\citealp{ImaiKeeleYamamoto10}). These assumptions may be challenging for some randomized experiment. The identification of the structural functions enables us to identify
\[
 y(1,d(1,\eta),U) - y(0,d(1,\eta),U)
\]
which is called the direct effect as opposed to the indirect effect
\[
 y(0,d(1,\eta),U) - y(0,d(0,\eta),U)
\]
in the literature of the mediation analysis (\citealp{Pearl09} and
\citealp{ImaiKeeleYamamoto10}). These quantities are useful when the policy has two stages $(T,D)$ whereas policymakers may consider forceful manipulation of the second stage $(D)$ which was not randomized in the experiment. Such motivation is the best
described in a dynamic treatment effect model (\citealp{Robins1986},
1987, \citealp{MurphyvanderLaanRobinsCPPRG01} or \citealp{Murphy03}). Consider a medical trial with initial randomized treatment and subsequent post-treatment medical treatment. In such a case, we need to know the net causal effects of both treatments since the manipulation of the second treatment is also a candidate treatment. For example, consider a medical trial of Swan-Ganz
Catheterization as studied in \cite{BhattacharaShaikhVytlacil12}. Such a treatment of Swan-Ganz Catheterization $T$ offers a criterion for doctors determining further medical treatment $D$. In this context, the
mediation effects are essential to the evaluation of the Catheterization
since both offering Catheterization $T$ and offering
post-Catheterization actions $D$ are manipulable, and essential for the evaluation of the effect of treatments $T$ and $D$ as a policy. Relevant parameters in such question require either exogenous
assignment of dynamic treatments (\citealp{Robins1986}, 1987,
\citealp{MurphyvanderLaanRobinsCPPRG01} or \citealp{Murphy03} in
Biostatistics under sequential randomization assumption), or a particular form of instruments as in Econometrics.\footnote{\cite{Han18} studies
identification of the dynamic treatment effects in the presence of an
instrument satisfying two-way exclusion
restrictions. \cite{HeckmanHumphriesVeramendi16} also studies
the dynamic treatment effects using conditional independence assumption or, instrumental variables.} While these parameters are out of scope
of this paper, my approach requires neither assumptions.
\end{comment}
